Accelerating Deep Convolutional Networks using low-precision and sparsity

We explore techniques to significantly improve the compute efficiency and performance of Deep Convolution Networks without impacting their accuracy. To improve the compute efficiency, we focus on achieving high accuracy with extremely low-precision (2-bit) weight networks, and to accelerate the execution time, we aggressively skip operations on zero-values. We achieve the highest reported accuracy of 76.6% Top-1/93% Top-5 on the Imagenet object classification challenge with low-precision network\footnote{github release of the source code coming soon} while reducing the compute requirement by ~3x compared to a full-precision network that achieves similar accuracy. Furthermore, to fully exploit the benefits of our low-precision networks, we build a deep learning accelerator core, dLAC, that can achieve up to 1 TFLOP/mm^2 equivalent for single-precision floating-point operations (~2 TFLOP/mm^2 for half-precision).

==> summary.tex <==
\section{Introduction}

\comment{case for specialization}
The two technology trends that result in the power wall are the nearly
constant per-transistor power requirements and fixed chip-level power budgets.
Hence, as the transistor density increases with each generation, so does the
fraction of the chip that is under-clocked or underused -- referred to as
\emph{dark silicon} -- due to the power concerns. In this regime, trading
the cheaper resource, dark silicon, for the more valuable resource, energy
efficiency, becomes a viable approach to scale system performance. The dark
silicon can be utilized to design specialized circuits that are significantly
more energy-efficient than general-purpose processors, and this approach
scales the system performance by allowing more computations to run in
parallel.

\comment{Challenges that specialization-based approaches bring for general-purpose domain}
Conventional accelerators reduce power for regular applications containing
ample data-level parallelism, but recent work~\cite{ccores} has
shown that specialized hardware can reduce power for irregular codes as well.
Moreover, these designs use specialized compute elements even for relatively
short running computations. This increases the fraction of program execution
on specialized, power-efficient hardware, but also raises questions about area
efficiency and re-usability, since each specialized core targets a very
specific computation. In addition, supporting a large number of tasks in
hardware would require designing a large number of specialized cores, which in
turn would make it difficult to tightly integrate all of them with the
general-purpose processor. Therefore, for specialization to be effective at
targeting a general-purpose system workload, the specialized processors must
ideally be able to support multiple computations, such that a relatively small
number of them can together support large fractions of system execution.

\comment{The \qasics\ enables the designer
to trade area for energy-efficiency in a scalable manner and can, when
combined, execute large portions of general purpose applications.}

\comment{Solution}


\comment{ provides energy-efficiency proportional to the area budget available
for specialization (shown in Figure~\ref{fig:areaPowerTradeoff})} 

\comment{QsCores introduction}

To trade silicon for specialization in a scalable manner, we propose a
new class of specialized processors,
\qasicexplNewLine. Unlike traditional ASICs, which target one specific task,
\qasics\ can support multiple tasks or computations. Because of this enhanced
computational power, a relatively small number of \qasics\ can potentially
support a significant fraction of a system's execution. Moreover, \qasics\ are
an order of magnitude more energy-efficient than general-purpose processors.
The \qasic\ design flow is based on the insight that ``similar'' code segments
exist within and across applications, and these code segments can be
represented by a single computation pattern. The \qasic\ design flow exploits
this insight by varying the required number of \qasics\ as well as their
computational power (i.e., the number of distinct computations they can
support) based on the relative importance of the applications and the area
budget available to optimize them. This enables \qasics\ to significantly
reduce the total area and the number of specialized processors compared to a
fully-specialized logic approach supporting the same functionality.

\comment{Contributions}

The goal of this work is to bring the benefits of specialization-based
approaches to the general class of irregular integer applications. In this
regard, we make the following contributions:

\begin{enumerate}

    \item \textbf{Configurable Compute Elements} \qasics\ enhance the
    computational power of specialized processors such that a relatively few
    of them, combined, can support a significant fraction of a system's
    execution. By doing so, \qasics\ make the specialization-based approaches
    more scalable by limiting the required amount of specialized logic.
    
     \item \textbf{Backward Compatibility} \qasics\ allow system designers to
    target the latest application versions while continuing to ably support
    the older ``in-use'' versions. This is a desirable quality because for
    many general-purpose applications, older versions are typically still be
    in use even though newer versions are available.
    
     \item \textbf{Application Re-targeting} The \qasic\ back-end compiler
    automatically retargets the application to benefit from any specialization
    available on the end-user system and it does so without any programmer
    feedback. This compiler support allows the current day applications to
    benefit from the new hardware features as and when they come out, without
    any software re-implementations and also, ensures that heterogeneity does
    not complicate software design.

\end{enumerate}


\comment{Results}

We evaluate \qasicP\ ability to target both a single application
library (e.g., data structures) as well as a diverse workload
consisting of applications selected from different domains
(e.g., SPECINT, EEMBC, and Vision). Our results show that
\qasics\ can provide 18.4$\times$ better energy efficiency than
general-purpose processors while reducing the amount of specialized
logic required to support the workload by up to 66\%.



\section{Overview}

This section overviews the design methodology of an \qasic-enabled system and evaluates its performance/energy efficiency.

\subsection{\qasicSubHeader-Enabled Systems}

The design flow of a \qasic-enabled system begins with a set of applications
that make up a significant fraction of the processor's target workload. We
profile these applications to extract the frequently used code segments,
called hotspots, which have high application coverage. The \qasic\ design flow
uses these hotspots to design specialized cores based on the area available
for specialization as well as the relative execution coverage of these
hotspots. The final step integrates these \qasics\ with a general-purpose
processor to build a heterogeneous tile. In the general case, a \qasic-enabled
system will consist of multiple heterogeneous tiles, each comprising several
\qasics\ targeting different workloads.

\boldparagraph{\qasic\ design flow} \qasic\ design flow is based on the insight that similar code patterns are present within and across applications. To exploit available similarity, our toolchain designs a computation pattern that encompasses these similar code structures and builds a \qasic\ for that computation pattern. 

The design flow accepts as input the hotspot functions as well as the area
budget available for specialization and generates a set of \qasics\ that
implement these hotspots and fit within the area budget. The design flow
starts by constructing a dependence graph corresponding to each of the hot
code segments. At each stage, the toolchain selects a dependence graph pair
that has similar code patterns present across them, uses these similar code
patterns to design a new dependence graph that represents both of the input
dependence graphs. It then replaces the input dependence graph pair with the
new merged graph. This process continues until the toolchain is unable to find
similar code segments across the dependence graphs or the area budget goals
are met.


This paper address the following challenges involved in implementing the
\qasic\ design flow mentioned above. The first challenge lies in identifying
similar code patterns across a wide range of general-purpose applications. The
hotspots of a typical general-purpose application tend to be many 100s of
instructions long and contain complex control-flow and irregular memory access
patterns, making the task of finding similarity both computationally intensive
and algorithmically challenging. The second challenge lies in exploiting these
similar code patterns to reduce hardware redundancy across specialized cores
by designing generalized code-structures that can execute all these similar
code patterns. The final challenge involves making the right area-energy
tradeoffs to ensure that the \qasics\ fit within the area budget, while
minimally impacting their energy efficiency. Addressing this challenge
requires finding efficient heuristics that approximate an exhaustive search of
the design space but avoid the exponential cost of that search.

\cfigure[data/areaPowerTradeoffGraph.pdf,{\figtitle{Effectiveness of \qasics\ vs.~ASICs as the area available for specialization varies}},fig:areaPowerTradeoff]

\subsection{Application compilation and runtime execution} 

The \qasic\ compiler automatically retargets application code to benefit from
all the specialized cores available without any programmer intervention. At
runtime, an application's execution migrates between the general-purpose
processor and \qasics\ based on whether a matching \qasic\ exists. This
execution migration is possible because of the tight coupling of \qasics\ and
the general-purpose processor via sharing of the L1 data cache and support for
arbitrary control transitions between the \qasic\ and the CPU.


\subsection{Results}

Figure~\ref{fig:areaPowerTradeoff} shows how the system's energy efficiency
varies with the area available for specialization for the hotspots of a
workload consisting of applications selected from various domains (including
SPECINT, EEMBC, Sat Solver, and Vision). The results show that our toolchain
can maintain high execution coverage (and hence high energy efficiency) even
when the area budget decreases by varying the computational power of \qasics.
In this case, \qasics\ provide $3\times$ more energy efficiency than
fully-specialized logic.


\vspace{-2mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%BIT BUCKET%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> texfooter.tex <==
  %%%%%%%%%%%%%%%%%%%%%%%%5
%\clearpage
%\pagestyle{empty}
%\input{department}
%\clearpage




%\bibliography{ws1,ws2,asplos,fpga,full,hot-chips,immd4,microchip,other,BuildingStuff}

%%\setstretch{0.75}
%%\titlespacing*{\section}{0em}{1ex}{1ex}
%\begin{small}

%\bibliographystyle{ieeetr}
%\begin{spacing}{0.3}
%\bibliographystyle{lib/bib/dj}  
%\bibliographystyle{abbrv}
%\bibliographystyle{mbt_dj}
%\bibliography{lib/bib/paper_abbrv,lib/bib/spe_abbrv}
%\bibliography{lib/bib/paper,lib/bib/spe}
%\end{spacing}
%\end{small}

%\clearpage
%\input{bio}
%\clearpage
%\input{budget}
%\clearpage
%\input{facilities}
\end{document}




==> texheader.tex <==
%\documentclass{sigplanconf}
%\documentclass[10pt,letterpaper,onecolumn]{article} 
\usepackage{pdfpages}
% The following \documentclass options may be useful:
%
% 10pt          To set in 10-point type instead of 9-point.
% 11pt          To set in 11-point type instead of 9-point.
% authoryear    To obtain author/year citation style instead of numeric.

\usepackage{setspace}
\usepackage{amsmath}
%\usepackage[usenames]{color}
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{url}
\urlstyle{rm}

%\usepackage[T1]{fontenc}
%\usepackage[scaled]{helvet}
%\renewcommand*\familydefault{\sfdefault} %% Only if the base font of the document is to be sans serif
%\usepackage{lmodern}
%\usepackage{ascii}

\usepackage{headers/tightenum}
\usepackage{multirow}

\usepackage[compact]{titlesec}

\pagestyle{empty} 
\pagenumbering{arabic}

\usepackage{textcomp}




\input{headers/macros}
\input{headers/defs}
%\newcommand{\ignore}[1]{}
\input{headers/remark}
%% Leave this on, so we can see them!!!
\remarktrue
\newcommand{\shortenum}{\vspace*{-0.1in}}
%\newcommand{\shortsec}{\vspace*{-0.2in}}
%\newcommand{\sparagraph}[1]{\vspace*{-0.2in}\paragraph{#1}}
%\newcommand{\sparagraph}[1]{\vspace*{-0.15in}\paragraph{#1}}
\newcommand{\sparagraph}[1]{\vspace*{0.0in}\paragraph{#1}}

% mbt: prevent figures on separate pages
\renewcommand{\textfraction}{0.1}


%\begin{document}
\pagestyle{empty} 
%\conferenceinfo{ASPLOS'10,} {March 13--17, 2010, Pittsburgh, Pennsylvania, USA.}
%\CopyrightYear{2010}
%\copyrightdata{978-1-60558-839-1/10/03}

%\titlebanner{banner above paper title}        % These are ignored unless
%\preprintfooter{short description of paper}   % 'preprint' option specified.

%\pagestyle{plain}


%\input{summary}
%\clearpage
%\pagestyle{myheadings}
%\pagenumbering{arabic}

%\newenvironment{smallitemize}{\begin{list}{$\bullet$}{\topsep0.0in\itemsep0.0in\parsep0.0in\partopsep0.0in\itemindent0.1in\leftmargin0.1in}}{\end{list}}
%\newenvironment{smallitemize}{\begin{list}{$\bullet$}{\topsep0.1in\itemsep0.1in\parsep0.1in\partopsep0.1in\itemindent0.1in\leftmargin0.1in}}{\end{list}}
%\newenvironment{smallitemize}{\begin{list}{$\bullet$}{\topsep0.05in\itemsep0.05in\parsep0.0in\partopsep0.05in\itemindent0.05in\leftmargin0.05in}}{\end{list}}
%{\topsep{0in}\itemsep{0.1in}\itemindent{0.1in}}
%%%%%%%%%%%%%%%%%%%%%%%%



